Dependency Parsing with the Structuralized Prompt Template

Dependency parsing is a fundamental task in natural language processing (NLP), aiming to identify syntactic dependencies and construct a syntactic tree for a given sentence. Traditional dependency parsing models typically construct embeddings and utilize additional layers for prediction. We propose a novel dependency parsing method that relies solely on an encoder model with a text-to-text training approach. To facilitate this, we introduce a structured prompt template that effectively captures the structural information of dependency trees. Our experimental results demonstrate that the proposed method achieves outstanding performance compared to traditional models, despite relying solely on a pre-trained model. Furthermore, this method is highly adaptable to various pre-trained models across different target languages and training environments, allowing easy integration of task-specific features.

==> table/PTB_data.tex <==
\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccc}
\hline
 &
  \begin{tabular}[c]{@{}c@{}}Data\\ Count\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Processed\\ Data Count\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Entries\\ Removed\end{tabular} \\ \hline
Dataset & \multicolumn{3}{c}{bg\_btb} \\ \hline
Train   & 39832     & 39829    & 3    \\ \hline
Dev     & 1700      & 1699     & 1    \\ \hline
Test    & 2146      & 2146     & 0    \\ \hline
\end{tabular}}

\caption{Data split for PTB dataset}
\end{table}

==> table/UD_data.tex <==
\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccc}

\hline
 &
  \begin{tabular}[c]{@{}c@{}}Data\\ Count\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Processed\\ Data Count\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Entries\\ Removed\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Data\\ Count\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Processed\\ Data Count\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Entries\\ Removed\end{tabular} \\ \hline
Dataset & \multicolumn{3}{c}{bg\_btb}    & \multicolumn{3}{c}{ca\_ancora}    \\ \hline
Train   & 8907      & 8907      & 0      & 13123       & 13087      & 36     \\ \hline
Dev     & 1115      & 1115      & 0      & 1709        & 1702       & 7      \\ \hline
Test    & 1116      & 1116      & 0      & 1846        & 1837       & 9      \\ \hline
Dataset & \multicolumn{3}{c}{cs\_pdt}    & \multicolumn{3}{c}{de\_gsd}       \\ \hline
Train   & 68495     & 68484     & 11     & 13814       & 13810      & 4      \\ \hline
Dev     & 9270      & 9269      & 1      & 799         & 799        & 0      \\ \hline
Test    & 10148     & 10146     & 2      & 977         & 977        & 0      \\ \hline
Dataset & \multicolumn{3}{c}{en\_ewt}    & \multicolumn{3}{c}{es\_ancora}    \\ \hline
Train   & 12543     & 12538     & 5      & 14305       & 14287      & 18     \\ \hline
Dev     & 2002      & 2002      & 0      & 1654        & 1653       & 1      \\ \hline
Test    & 2077      & 2077      & 0      & 1721        & 1717       & 4      \\ \hline
Dataset & \multicolumn{3}{c}{fr\_gsd}    & \multicolumn{3}{c}{it\_isdt}      \\ \hline
Train   & 14554     & 14542     & 12     & 13121       & 13098      & 23     \\ \hline
Dev     & 1478      & 1477      & 1      & 564         & 564        & 0      \\ \hline
Test    & 416       & 416       & 0      & 482         & 481        & 1      \\ \hline
Dataset & \multicolumn{3}{c}{nl\_alpino} & \multicolumn{3}{c}{no\_bokmaal}   \\ \hline
Train   & 12269     & 12269     & 0      & 15696       & 15696      & 0      \\ \hline
Dev     & 718       & 718       & 0      & 2410        & 2410       & 0      \\ \hline
Test    & 596       & 596       & 0      & 1939        & 1939       & 0      \\ \hline
Dataset & \multicolumn{3}{c}{ro\_rrt}    & \multicolumn{3}{c}{ru\_syntagrus} \\ \hline
Train   & 8043      & 8032      & 11     & 48814       & 48803      & 11     \\ \hline
Dev     & 752       & 750       & 2      & 6584        & 6579       & 5      \\ \hline
Test    & 729       & 724       & 5      & 6491        & 6490       & 1      \\ \hline
\end{tabular}}

\caption{Data split for UD2.2 dataset}
\end{table}
